Argus: From Rasterized-Camera Self-Play to Real-Camera Driving

Self-play reinforcement learning (RL) in simulation lets driving scale with compute rather than with logged human data, but learning from scratch takes billions of steps, so observations must be cheap to render. Rasterized camera views show what driving mostly depends on, the road, lanes, road users, and traffic lights, at a fraction of the cost of realistic images, and through a pretrained image encoder such as DINOv3, a real camera image resembles its raster. We present Argus, a camera policy that inherits all of its driving skills from Argus-Raster, a raster policy trained by self-play, interleaved toward the end of its training with single-agent PPO in logged scenes. Only its pretrained image encoder is aligned: it learns to match Argus-Raster's features on a raster twin of the scene, drawn from the perception labels that driving datasets provide. Its driving comes from 5M hours of RL in simulation, so Argus needs little camera data. Aligned on only 2.2 hours of reconstructed camera views of driving scenes, it already beats the best camera planner on AlpaSim PAI, a model trained on 1,800 hours of driving. Aligned on 25 hours of such views, Argus outperforms in closed loop on AlpaSim and HUGSIM every camera policy we compare with, learned by imitation or transferred from self-play, by 5.8 points on PAI and 4.9 on nuPlan, and Argus+, with a larger image backbone, is ahead of every planner it is compared with on AlpaSim, HUGSIM, NavSafe-$\infty$, and Odyssey, with 87.3 on PAI. Project page: https://valeoai.github.io/Argus

==> fig/architecture_detail.tex <==
\begin{figure*}[t]
  \centering
  \resizebox{\linewidth}{!}{%
\figfont
\includegraphics{fig/pdf/architecture_detail.pdf}}
  \caption{\textbf{Networks of \argusraster and \argus.}
    Top: the raster encoder $E$ of \argusraster. Bottom: the image encoder $E'$ of \argus, an image backbone $B$ and an adapter $A$.
    Right: the driving head $H$, shared by both and frozen in \argus; blue from the latents of \argusraster, orange from those of \argus.
    \argus is its image encoder $E'$ with $H$, and drives through the trajectory head of $H$; \argus w/~action drives through its action head.
    Dashed: the alignment losses.
    See \autoref{sec:impl:arch} for the blocks and their sizes.}
  \label{fig:architecture_detail}
\end{figure*}


==> fig/backbone_analysis.tex <==
\begin{figure*}[t]%
  \centering
  {\figfont
  \colorlet{dvtwocol}{black!55}%
  \colorlet{sigcol}{blue!60!black}%
  \colorlet{dacol}{teal!75!black}%
  \colorlet{pecol}{violet!70!black}%
  \colorlet{eupecol}{olive!75!black}%
  \colorlet{samcol}{brown!85!black}%
  \newcommand{\bbline}[2]{\foreach \m/\s [remember=\m as \bbpm (initially 0), remember=\s as \bbps (initially 0)] in {#2} {%
      \ifdim\bbpm pt>0pt \draw[#1, line width=0.9pt] ({log10(\bbpm)},\bbps) -- ({log10(\m)},\s);\fi}}%
  \newcommand{\bbdot}[3]{\node[circle, fill=#1, draw=white, line width=0.4pt, inner sep=1.7pt] at ({log10(#2)},#3) {};}%
  \newcommand{\bbstar}[2]{\node[star, star points=5, star point ratio=2.3, fill=arguscol, draw=white, line width=0.3pt, inner sep=0pt, minimum size=7.5pt] at ({log10(#1)},#2) {};}%
  \newcommand{\bblab}[7]{\draw[#1!70, line width=0.3pt] ({log10(#2)},#3) -- ({log10(#4)},#5);\node[text=#1, anchor=#6, font=\scriptsize\bfseries, inner sep=1.2pt] at ({log10(#4)},#5) {#7};}%
  \newcommand{\bbpanel}[6]{%
    \foreach \g in {#3} {\draw[black!10, line width=0.3pt] (0.6,\g) -- (2.2,\g); \node[text=black!55, anchor=east, inner sep=1.5pt] at (0.6,\g) {\g};}%
    \draw[black!40, line width=0.4pt] (0.6,#2) -- (2.2,#2);
    \foreach \m in {5,10,20,50,100} {\pgfmathsetmacro{\lgx}{log10(\m)}\draw[black!40, line width=0.4pt] (\lgx,#2) -- ++(0,-0.065cm);
      \node[text=black!55, anchor=north, inner sep=1pt] at ([yshift=-0.08cm]\lgx,#2) {\m M};}
    \node[anchor=south west, text=black!65, inner sep=0.5pt] at ([yshift=0.1cm]0.42,#6) {#4};
    \draw[enccol, dash pattern=on 2.5pt off 1.5pt, line width=0.7pt] (0.6,#5) -- (2.2,#5);}%
  \includegraphics{fig/pdf/backbone_analysis.pdf}}
  \DeclareRobustCommand{\bbmklink}{\tikz[baseline=-0.6ex]\draw[arguscol, line width=0.9pt, dash pattern=on 2pt off 1.2pt] (0,0) -- (0.45cm,0);}%
  \DeclareRobustCommand{\bbmkstar}{\tikz[baseline=-0.6ex]\node[star, star points=5, star point ratio=2.3, fill=arguscol, inner sep=0pt, minimum size=7pt]{};}%
  \DeclareRobustCommand{\bbmkref}{\tikz[baseline=-0.6ex]\draw[enccol, dash pattern=on 2.5pt off 1.5pt, line width=0.7pt] (0,0) -- (0.45cm,0);}%
  \caption{\textbf{Image backbone}: AlpaSim scene score of \argus aligned with image backbones of several families and sizes, on (a) the nuPlan track and (b) the PAI track, against their number of parameters.
    A line links the models of one family; \bbmklink: the ViT-T/16 that Lightly distills from DINOv3 ViT-L/16; \bbmkstar: the default; \bbmkref: \argusraster.}%
  \label{fig:backbone_analysis}
\end{figure*}


==> fig/data_source.tex <==
\begin{figure}[t]
  \centering
  \resizebox{\linewidth}{!}{%
\figfont
\includegraphics{fig/pdf/data_source.pdf}}
  \caption{\textbf{Collection of the alignment data}: AlpaSim scene score of \argus aligned for the same number of steps on frames of the logged human drives, of the drives of \argusraster that score 1 (default, orange, $^{\star}$) or of all of them, or of both.
    Gray segments link each score to the default.}
  \label{fig:data_source}
\end{figure}


==> fig/selfplay_scaling.tex <==
\def\sclpai{3.595/25.17/south east,10.300/48.82/south east,20.641/54.61/south east,41.489/57.43/south,50.586/55.97/north east}%
\def\sclpaidecay{50.586/55.97/61.268/61.1/south}%
\begin{figure}[t]%
  \centering
  {\figfont
  \pgfmathdeclarefunction{sclxf}{1}{\pgfmathparse{(log10(#1)-log10(3))*65/(log10(70)-log10(3))}}%
  \newcommand{\sclx}[1]{sclxf(#1)}%
  \newcommand{\sclpanel}[8]{%
    \begin{scope}[xshift=#1cm, yshift={-#2*#5*1cm}, y=#5cm]%
      \foreach \g in {#4} {\draw[black!10, line width=0.3pt] (0,\g) -- (65,\g);
        \node[text=black!55, anchor=east, inner sep=1.5pt] at (0,\g) {\g};}
      \draw[black!40, line width=0.4pt] (0,#2) -- (65,#2);
      \foreach \s in {3,5,10,20,50} {\pgfmathsetmacro{\tx}{\sclx{\s}}\draw[black!40, line width=0.4pt] (\tx,#2) -- ++(0,{-0.08/#5});
        \node[anchor=north, inner sep=1pt] at (\tx,{#2-0.1/#5}) {\s};}%
      \node[anchor=south west, text=black!65, inner sep=0.5pt] at ([yshift=0.1cm]-6,#3) {#6};%
      \foreach \p/\s/\a [remember=\p as \tpp (initially -1), remember=\s as \tps (initially 0)] in #7 {%
        \ifdim\tpp pt>-1pt \pgfmathsetmacro{\txa}{\sclx{\tpp}}\pgfmathsetmacro{\txb}{\sclx{\p}}\draw[enccol, line width=1pt] (\txa,\tps) -- (\txb,\s);\fi}%
      \foreach \p/\s/\a in #7 {%
        \pgfmathsetmacro{\tx}{\sclx{\p}}%
        \node[circle, fill=enccol, draw=white, line width=0.4pt, inner sep=1.8pt] at (\tx,\s) {};
        \pgfmathsetmacro{\tpl}{round(10*\s+0.01)/10}%
        \node[anchor=\a, inner sep=2.5pt, text=enccol, font=\scriptsize\bfseries] at (\tx,\s) {\pgfmathprintnumber[fixed, precision=1, fixed zerofill, assume math mode=true]{\tpl}};}%
      \foreach \xa/\ya/\xb/\yb/\a in #8 {%
        \pgfmathsetmacro{\txa}{\sclx{\xa}}\pgfmathsetmacro{\txb}{\sclx{\xb}}%
        \draw[black!45, line width=0.6pt, dash pattern=on 2pt off 1.5pt] (\txa,#2) -- (\txa,#3);%
        \node[rotate=90, anchor=north west, inner sep=1.5pt, text=black!55, font=\tiny] at (\txa,#2) {LR decay};
        \draw[enccol, line width=1pt] (\txa,\ya) -- (\txb,\yb);
        \node[circle, fill=enccol, draw=white, line width=0.4pt, inner sep=1.8pt] at (\txb,\yb) {};
        \pgfmathsetmacro{\tpl}{round(10*\yb+0.01)/10}%
        \node[anchor=\a, inner sep=2.5pt, text=enccol, font=\scriptsize\bfseries] at (\txb,\yb) {\pgfmathprintnumber[fixed, precision=1, fixed zerofill, assume math mode=true]{\tpl}};}%
    \end{scope}}%
  \includegraphics{fig/pdf/selfplay_scaling.pdf}}
  \caption{\textbf{Scaling self-play}: AlpaSim PAI score of the self-play policy, \argusraster after self-play only and driving with its action head, against the number of self-play steps (B: billions).}%
  \label{fig:selfplay_scaling}
\end{figure}


==> fig/trajectory_head.tex <==
\begin{figure}[t]
  \centering
  \resizebox{\linewidth}{!}{%
\figfont
\includegraphics{fig/pdf/trajectory_head.pdf}}
  \caption{\textbf{Trajectory head.}
    Top: the frozen action head (blue) drives for 3.9\,s, then the trajectory head (purple) for 2.1\,s; the target of a state is the path the action head then drives, a recovery (shaded) from a state $s$ the trajectory head reached.
    Bottom: from the frozen features and the chosen action, the trajectory head learns by flow matching to turn noise into the target poses.}
  \label{fig:trajectory_head}
\end{figure}


==> sec/A_implementation.tex <==
\section{Implementation details}
\label{sec:impl}

\argusraster learns to drive by self-play in a simulator that renders what each agent's cameras see as raster views (\autoref{sec:impl:sim}), rewarded as in \autoref{sec:impl:selfplay}, with one network that reads any camera rig (\autoref{sec:impl:arch}).
Self-play is then extended to logged scenes, where the same network learns to drive among recorded traffic (\autoref{sec:impl:logged}), and the network gains a trajectory head that plans (\autoref{sec:impl:traj}).
\argus keeps all of it and only replaces the raster encoder with an image encoder, aligned on camera frames (\autoref{sec:impl:align}).

\subsection{Simulator}
\label{sec:impl:sim}

\paragraph{Scenes.}
A scene places agents on one of the 12 maps of self-play and draws at random its traffic density, its speed limits and its parked cars, so that self-play meets traffic from empty roads to dense crowds.
The number of agents of each type is its density times the lane length of the map.

A scene holds up to 300 agents, spawned in one region of the map.
Most of them are vehicles, whose density is drawn from a mixture of regimes that averages about 10 vehicles per lane-kilometer and reaches 30.
Pedestrians and cyclists follow regimes of their own, averaging 0.95 and 0.9 per lane-kilometer, so that about one agent in ten is a pedestrian.
Pedestrians walk in groups along the curbs and cross the road at their turn-arounds.
In half of the scenes, the speed limits of the lanes, which vehicles and cyclists follow, are scaled by a factor drawn between 0.6 and 1.6.
Parked cars line the road edges at about 10 per kilometer of curb, and 30\% of their clusters straddle the curb.
The goals of a route are waypoints 20 to 60\,m apart.

\paragraph{Motion model.}
Every agent, whether vehicle, cyclist or pedestrian, moves by the same model. As in Gigaflow~\cite{cusumanotowner2025gigaflow}, an action $(j_\text{long}, j_\text{lat})$, a longitudinal and a lateral jerk, is integrated once per policy step $\Delta t$, where a superscript $+$ marks a value after the step,
\begin{align*}
  a_\text{long}^{+} &= \mathrm{clip}\big(a_\text{long} + c_\mathrm{throttle}\, j_\text{long}\, \Delta t,\; -5,\; 2.5\, c_\mathrm{acc}\big), \\
  a_\text{lat}^{+} &= \mathrm{clip}\big(a_\text{lat} + c_\mathrm{steer}\, j_\text{lat}\, \Delta t,\; -4,\; 4\big), \\
  v^{+} &= \mathrm{clip}\big(v + \tfrac{1}{2}(a_\text{long} + a_\text{long}^{+})\,\Delta t,\; -2,\; v_\mathrm{max}\big),
\end{align*}
with accelerations in m/s$^2$ and speeds in m/s; an acceleration or a speed that would change sign is set to zero instead, and a stop also resets both accelerations.
The lateral acceleration sets a target steering angle on the wheelbase $L$, which is 0.6 times the agent's length,
\begin{align*}
  \delta^\star &= \arctan\!\Big(\frac{a_\text{lat}^{+}\, L}{\max(|v^{+}|, 1)^2}\Big), \\
  \delta^{+} &= \mathrm{clip}\big(\delta + \mathrm{clip}(\delta^\star - \delta,\, \pm\dot\delta_\mathrm{max}\Delta t),\, \pm\delta_\mathrm{max}\big),
\end{align*}
with $\dot\delta_\mathrm{max} = 0.6$\,rad/s and $\delta_\mathrm{max} = 0.55$\,rad.
The agent then moves along the arc of curvature $\kappa = \tan\delta^{+} / L$: over the distance $\ell = \tfrac{1}{2}(v + v^{+})\,\Delta t$, its heading $\psi$ and position $(x, y)$ change by
\begin{align*}
  \Delta\psi &= \kappa\,\ell, \\
  \Delta x_\mathrm{loc} &= \frac{\sin\Delta\psi}{\kappa}, \qquad
  \Delta y_\mathrm{loc} = \frac{1 - \cos\Delta\psi}{\kappa}, \\
  \Delta x &= \Delta x_\mathrm{loc}\cos\psi - \Delta y_\mathrm{loc}\sin\psi, \\
  \Delta y &= \Delta x_\mathrm{loc}\sin\psi + \Delta y_\mathrm{loc}\cos\psi,
\end{align*}
in the agent's frame and then in the world frame, with $(\Delta x_\mathrm{loc}, \Delta y_\mathrm{loc}) = (\ell, 0)$ on a straight path.
The speed cap $v_\mathrm{max}$ and the multipliers $c_\mathrm{throttle}$, $c_\mathrm{steer}$, and $c_\mathrm{acc}$ are drawn per agent as in \autoref{tab:selfplay_rewards}.

\paragraph{Cameras.}
Each agent receives the raster views of its own camera rig, and vehicles carry the rigs of real cars.
In self-play, a vehicle draws its rig among the rigs of the pool: a default rig, the rigs of nuPlan and nuScenes, the rigs of the four datasets of HUGSIM (nuScenes, PandaSet, KITTI-360, and Waymo), and the three rigs of the PAI track of AlpaSim, which leave out their 30$^\circ$ telephoto camera.
The nuScenes rig of HUGSIM differs from the calibrated rig of nuScenes: HUGSIM renders the same cameras levelled, 0.3\,m lower, and around an origin under the front camera.
These rigs give only the placement and the lenses of the cameras, through which the simulator renders its own scenes; see \autoref{sec:impl:logged} for the rigs of the training extension.
Each rig is attached at the rear axle of the vehicle, and its cameras keep the offsets and heights from the rear axle that they have on the source car; the ray codes follow these cameras.
For simplicity, pedestrians and cyclists see through four cameras around them, tilted 15$^\circ$ downward, which is enough for them to move reliably among the vehicles; a more realistic model of their perception is left for future work.

\subsection{Self-play training}
\label{sec:impl:selfplay}

\paragraph{Rewards.}
\input{tab/selfplay_rewards}
The rewards follow those of Gigaflow~\cite{cusumanotowner2025gigaflow}.
A vehicle is paid for reaching the waypoints of its route, punished for the events that end a drive, and shaped by small dense terms that keep it in its lane, comfortable, within the speed limit, and moving.
At each policy step $\Delta t$, a vehicle receives the sum of five terms, with the coefficients $\alpha$ of \autoref{tab:selfplay_rewards},
\begin{equation*}
  r = r_\mathrm{goal} + r_\mathrm{event} + r_\mathrm{lane} + r_\mathrm{comf} + r_\mathrm{motion}.
\end{equation*}
The goal term pays the route,
\begin{equation*}
  r_\mathrm{goal} = n_\mathrm{goal},
\end{equation*}
where $n_\mathrm{goal}$ counts the route waypoints reached within $\delta_\mathrm{goal}$ in the step, and the last one counts only when it is reached below the speed $v_\mathrm{goal}$.
The event term punishes the events that end a drive,
\begin{align*}
  r_\mathrm{event} = {} & -\big(\alpha_\mathrm{coll} + 0.1\,|v|\big)\,\mathbf{1}_\mathrm{coll} \\
  & - \alpha_\mathrm{off}\,\mathbf{1}_\mathrm{off} - \alpha_\mathrm{stop}\,\mathbf{1}_\mathrm{stop},
\end{align*}
where the indicators mark a collision, leaving the road, and running a red light or a stop sign, and where $v$ is the signed speed in m/s: the collision penalty grows with its magnitude, so that a collision costs more the faster it happens.
The lane term keeps the vehicle in its lane, $r_\mathrm{lane} = r_\mathrm{align} + r_\mathrm{center}$, with
\begin{align*}
  r_\mathrm{align} &= \alpha_\mathrm{align}\,\Delta t\,\big[\min(\cos\theta, 0) + \alpha_\mathrm{wrong}\min(v\cos\theta, 0) \\
  &\qquad + 0.0025\,\big(1 - \tfrac{2|\theta|}{\pi}\big)\big], \\
  r_\mathrm{center} &= -\alpha_\mathrm{center}\,\Delta t\,\big[\mathbf{1}_\mathrm{aligned}\,|d - b| - 0.05\,e^{-(|d-b|-0.5)}\big],
\end{align*}
where $\theta$ is the angle between the vehicle's heading and its lane and $d$ its lateral offset from the lane center: $r_\mathrm{align}$ penalizes facing or driving against the lane and slightly rewards facing along it, while $r_\mathrm{center}$, applied when the vehicle is aligned with its lane, penalizes its offset from the lane center shifted by the bias $b$.
The comfort term keeps the drive smooth and within the speed limit,
\begin{equation*}
  r_\mathrm{comf} = -\alpha_\mathrm{comf}\, n_\mathrm{comf} - \alpha_\mathrm{over}\,\mathbf{1}_\mathrm{over},
\end{equation*}
where $n_\mathrm{comf}$ counts the longitudinal and lateral accelerations above 3\,m/s$^2$ and the longitudinal or lateral jerks above 5\,m/s$^3$, and $\mathbf{1}_\mathrm{over}$ marks a speed more than 2\,m/s above the lane's limit.
The motion term rewards progress and penalizes reversing and idle activity,
\begin{align*}
  r_\mathrm{motion} = {} & \alpha_\mathrm{prog}\,\Delta t\,\mathbf{1}_{v > 2.5}\max(\cos\theta, 0) \\
  & - \alpha_\mathrm{rev}\,\Delta t\,\mathbf{1}_{v < 0} - \alpha_\mathrm{time}\,\Delta t\,\mathbf{1}_\mathrm{active},
\end{align*}
where $\mathbf{1}_\mathrm{active}$ marks every step in which the vehicle moves or accelerates.
Compared with Gigaflow, the goal speed is drawn per agent instead of fixed at 3\,m/s, the overspeed penalty is added, stop signs are penalized like red lights, and pedestrians receive only the goal and collision terms, with a smaller goal radius and goal speed than vehicles.
At every spawn, each agent draws its coefficients, three dynamics multipliers and a speed cap, all of which the policy observes, so that a single network drives with many personalities, and they are fixed to the Eval column of \autoref{tab:selfplay_rewards}.

\paragraph{Training.}
Every agent of every environment drives with the same network, and PPO~\cite{schulman2017ppo} trains it on the experience of all of them, gathered on 260 A100 GPUs.
The learning rate stays constant at $5\cdot10^{-4}$ for 50B agent steps and then decays to zero over 10B more steps, and \autoref{tab:selfplay_hparams}a gives the other hyperparameters.

\subsection{Base architecture}
\label{sec:impl:arch}

\input{fig/architecture_detail}

Self-play trains the base network of the policy, which every agent runs on its own raster views and which outputs one action per step: a raster encoder $E$ and a driving head $H$ with an action head and a value head.
The later stages keep this network and add to it, a trajectory head in $H$ that plans (\autoref{sec:impl:traj}) and, for \argus, an image encoder $E'$ in place of $E$ (\autoref{sec:impl:align}).
\autoref{fig:architecture_detail} shows all of them, and this section describes the base network.

\paragraph{Raster encoder.}
The raster encoder $E$ reads the raster views in two stages: a raster backbone $C$ summarizes each camera, and a scene pooler $P$ gathers the summaries of all cameras into 32 latents.
The raster backbone $C$ summarizes each camera into a few tokens and tells them where the camera looks, so that the same weights read any rig.
Each $96{\times}54$ view is zero-padded at the bottom to $96{\times}56$, so that no row is dropped, and cut into $12{\times}7$ patches of $8{\times}8$ pixels that are embedded to width 128; every attention block has 4 heads, an MLP ratio of 4 and GELU activations.
Each patch token carries a code of its viewing ray, which tells it both where it sits in the image and where its camera is mounted and looks: the ray through the center of the patch is written in the ego frame by its Pl\"ucker coordinates, a direction and a moment, and encoded by sines and cosines at ten frequencies, as a positional encoding.
Two self-attention blocks run within each camera.
From the first block on, the patch tokens of each camera are joined by 16 summary tokens.
These are learned queries shared by all cameras and shifted for each camera by an MLP of its mean ray code, and only the summaries leave the encoder.
The adapter of the alignment, described in \autoref{sec:method:alignment}, maps onto these summary tokens of width 128.
The scene pooler $P$ compresses the summaries of all cameras into the 32 latents with one cross-attention block, and reads only these image tokens.

\paragraph{Driving head.}
The driving head $H$ turns the 32 latents into an action and a value.
Its trunk, a transformer of four blocks, runs over the latents together with the tokens of the ego state and of the conditioning vector, which also carries the three goals, and in its last block eight action and eight value read-out tokens attend to all of them.
A linear action head maps the eight action read-outs ($8{\times}128$ values) to the 12 jerk actions of \autoref{sec:method:training}, and a linear value head maps the eight value read-outs to the value, so that the actor and the critic share the whole network.
All transformer blocks of the network, in the raster backbone, the scene pooler, and the trunk, use the gating of GTrXL~\cite{parisotto2020gtrxl}.
Of these two heads, the action head drives and the value head serves the value loss of the alignment; the trajectory head of \autoref{sec:impl:traj}, added to $H$ after RL training, drives by default.

\subsection{Extending self-play to logged traffic}
\label{sec:impl:logged}
\input{tab/training_settings}%
Driving tasks are often defined on logged scenes~\cite{caesar2021nuplan,dauner2024navsim,zhou2026hugsim}: a scene comes with its recorded road users, a route, and the conditions that end a drive.
The training extension brings such scenes into the simulator of \autoref{sec:impl:sim}: it keeps the network of \autoref{sec:impl:arch}, the PPO trainer, and most reward terms of self-play, and adapts four things to the logged scenes: the scenes themselves, the motion of the ego, its observations, and the termination conditions.
\autoref{tab:logged_hparams}a gives its settings beside those of self-play.

\paragraph{Scenes.}
The ego drives among the recorded road users of the logged scenes of the two AlpaSim tracks, the PAI training scenes and the navtrain road blocks, so that it learns the human traffic of the logs.
Of the 1{,}761 PAI training scenes, 300 are kept out of training, the training held-out scenes, to choose checkpoints and settings, and 3 whose logged drive leaves the road are dropped.
The environments that run logged scenes draw the PAI scenes with weight 1 and the navtrain scenes with weight 0.28.

\paragraph{Motion of the ego.}
Many driving stacks move the car through a controller that tracks a planned trajectory rather than through the policy's own commands, and the extension uses one such controller throughout, the linear MPC and vehicle model of AlpaSim.
Each jerk step of the policy is turned into a short plan, through inverse dynamics and an inverted linear MPC, which the controller then tracks, with the rear-axle offset of the scene.
The policy thus learns the motion that its actions produce in the logged scenes rather than in self-play.

\paragraph{Observations.}
In 70\% of the episodes, a scene is rendered with the camera rig of its own car, which for navtrain is the rig of the nuPlan track.
In the others, it is rendered with one of the other rigs of the pool of \autoref{sec:impl:sim}, so that the policy keeps reading rigs other than those of the logged scenes.
AlpaSim's ego hood covers part of the front camera, and in half of the episodes this part is rendered as empty background.
Every lane shows a speed limit of 40\,m/s.
At each step, the pose of the ego receives Gaussian noise of 8\,cm and $1^\circ$.
The log drives the ego through a short warm-up before handing it over.

\paragraph{Termination conditions and reward.}
The termination conditions are those of the task, and the coefficients of the terminal events are fixed to their values in the Eval column of \autoref{tab:selfplay_rewards}, while the others are still drawn per agent.
A contact counts as being rear-ended when the other car's box touches the ego's rear bumper and not its front one; it then costs $-0.5$ and ends the episode.
The neural reconstructions of a logged scene degrade away from its recorded path, so a drive must stay within a corridor of 4\,m on each side of that path, as defined in \autoref{sec:protocol:benchmarks}.
The extension enforces it with $r_\mathrm{corridor} = -0.25\,\Delta t\,\max(d - 2,\, 0)$ per step of $\Delta t$ seconds, where $d$ is the lateral distance in meters of the ego from the recorded path, and ends the drive with a reward of $-3$ once $d$ reaches 4\,m, as if it left the road.
This term is a constraint of the reconstruction, not a pull toward the log.
Within 2\,m of the corridor's center, no term acts, so the ego chooses its own speed, timing and position there.
The goals are three waypoints 20 to 60\,m apart on the ego's logged route, which is extended 120\,m along the lanes past the end of the log as AlpaSim's route is, and a goal that the ego passes without reaching it is skipped.

\paragraph{Training.}
The run starts from the self-play policy and trains in two worlds at once: two of the eight environments of each GPU keep running the self-play world of \autoref{sec:impl:selfplay}, at the step of the extension, so that the policy does not forget self-play, and the other six run the logged scenes.
Each world normalizes its advantages separately and has its own linear value head on the shared trunk; only the value head of the logged scenes is kept after training, and it is the value head $V$ that the alignment matches (\autoref{sec:impl:align}).
It runs for 342M steps, a quarter of them in the self-play world, in about 4\,h on 8 H100 GPUs, 32 H100 GPU-hours, and \autoref{tab:logged_hparams}a gives its hyperparameters.

\subsection{Trajectory head by online self-distillation}
\label{sec:impl:traj}

\input{fig/trajectory_head}
After RL training, a trajectory head learns to plan on the frozen network, with the action head of the same network as its only expert.
The encoders, the trunk and the action head keep their weights, and both heads read the same features.

\paragraph{Head architecture.}
The head generates a plan of 10 poses by rectified flow matching~\cite{liu2023rectifiedflow}, conditioned on the scene and on the action chosen by the action head.
Its denoiser is a transformer of about 2.0M parameters with four blocks of width 128 and four attention heads.
In each block, the 10 pose tokens attend to each other and then to the scene before an MLP; adaptive layer normalization modulates all three, and the output layer of each block starts at zero.
The scene is made of the action read-out of the network, its 32 latents, and its ego and conditioning tokens.
The modulation encodes the flow time, the action read-out and an action.
In training, this action is the one that the action head executed, replaced by a null class for 15\% of the samples, and at deployment it is the most likely action of the action head.
The flow time is drawn from a logit-normal distribution, and the loss is the squared error of the predicted velocity over the valid poses.

\paragraph{Rollouts.}
The head needs no dataset: it learns from the drives that the policy makes while the head trains, with no replay buffer.
The policy is the one extended to logged traffic, frozen, and it drives the ego in the logged scenes only, without the self-play world, at a simulator step of 0.1\,s.

\paragraph{Handover.}
As in DAgger~\cite{ross2011dagger}, the two heads take turns driving the ego, in the cycle at the top of \autoref{fig:trajectory_head}.
The action head drives for 39 steps (3.9\,s), with its most likely action at every step.
It then hands the ego over to the trajectory head, which drives the next 21 steps (2.1\,s): at every step, it plans again from the current state, and AlpaSim's linear MPC tracks the latest plan.
The action head then takes over from the state $s$ that the trajectory head reached, so the path that it drives from $s$ recovers from the errors of the trajectory head, and this path becomes a target of the trajectory head.
The cycle repeats every 60 steps, and the trajectory head drives about a third of them.
At the start of training, the trajectory head takes over at a handover only with a probability that rises linearly from 0 to 1 over the first 2\% of training; otherwise the action head keeps driving.

\paragraph{Targets.}
The trajectory head learns to predict the path that the action head drives.
At a step where the action head drives, the target is the path of the ego over the next 3\,s of the same rollout, as 10 poses 0.3\,s apart, each given in the ego frame as its normalized increment $(\Delta x, \Delta y, \cos\Delta\theta-1, \sin\Delta\theta)$.
If the trajectory head takes over within these 3\,s, the target stops at the handover, and its later poses are left out of the loss.
Steps where the trajectory head drives give no target, and neither do steps whose next 3\,s end in a failure that ends the episode; in these rollouts, a contact or leaving the road does not end the episode.

\paragraph{Training.}
The head trains on this frozen policy, on each step with a target once, in the epoch that collected it.
During training, the trajectory head samples each plan from Gaussian noise in a single Euler step.
It runs for 256M steps in the logged scenes, in about 4\,h on 8 H100 GPUs, 32 H100 GPU-hours, and \autoref{tab:selfplay_hparams}b gives its hyperparameters.

\subsection{Alignment to camera images}
\label{sec:impl:align}

The alignment trains the image encoder $E'$ of \argus, which consists of an image backbone $B$ and an adapter $A$ whose last part is a trainable copy of the scene pooler $P$, so that on each frame its latents and the outputs of the frozen head match those that \argusraster produces on the raster twin of the frame.

\paragraph{Data.}
\label{sec:impl:align_data}
Each sample of the alignment is a frame of a drive in a reconstructed scene, with its camera views, its vector $\mathbf{s}$ of ego state and conditioning, and its raster twin.

\emph{Collection method.}
The alignment uses camera views of the states that the policy itself visits: \argusraster drives reconstructed driving scenes in AlpaSim, which renders the camera views along each drive.
Only scenes released for training are driven: the 1{,}761 training scenes of PAI, reconstructed by NuRec, and the 12{,}861 road blocks of navtrain~\cite{dauner2024navsim}, one 5\,s scene each, reconstructed in WorldEngine~\cite{li2026worldengine} by MTGS~\cite{li2025mtgs}.
\argusraster drives them with its action head, with the driver and settings of \autoref{sec:protocol:ours} otherwise, for about 9.7\,h and 17.8\,h of driving.
Only the drives that it completes with a score of 1 are kept, those of 1{,}579 PAI and 11{,}607 navtrain scenes, 8.7\,h and 16.1\,h of driving, at one frame per policy step of 0.1\,s.

\emph{Frames.}
Each frame holds the views of the cameras of its own car, listed in \autoref{tab:align_hparams}c.
Each frame also stores the vector $\mathbf{s}$ that both policies read, filled from the drive: the recorded motion of the ego (speed, steering angle, and accelerations), the fixed conditioning vector (Eval column of \autoref{tab:selfplay_rewards}), the three goals on the route of \autoref{sec:protocol:benchmarks}, and the speed limit of 40\,m/s.
The ray codes follow each camera's calibration, so that one camera policy reads rigs of different layouts.

\emph{Raster twins.}
Each frame is paired with its raster twin, the raster views that the frozen \argusraster read at that step of the drive, so that \argusraster gives on it the action and the value that the camera policy is aligned to.
Rebuilt from the recorded drive, its raster views draw the map of the scene, the recorded road users and the ego, at $96{\times}54$ pixels with the ego hood, through the cameras of the frame: on PAI, the five f-theta cameras of the nearest PAI rig, without the telephoto camera, and on navtrain, the four nuPlan cameras.

\paragraph{Image encoder.}
The image encoder $E'$ reads each camera with an image backbone $B$, a DINOv3 ViT-S/16~\cite{simeoni2026dinov3} adapted by LoRA~\cite{hu2022lora}, which reads the geometry of the camera through ray codes, as the raster backbone $C$ does: the ray code of each patch is added to its patch token, and the ray code of the camera shifts its scene tokens, both through projections initialized to zero and trained with the LoRA.
An adapter then maps the 16 scene tokens of each camera onto the 16 summary tokens of \argusraster for that camera, as the sum of a linear map per token slot, initialized at random, and a two-layer transformer over the tokens of all cameras, initialized to zero, so that the adapter starts as the linear map alone (\autoref{fig:architecture_detail}, bottom).
The last part of the adapter, a trainable copy of the scene pooler $P$ of \argusraster, turns them into the 32 latents that its frozen head reads.

\paragraph{Losses.}
This paragraph details the three losses of \autoref{sec:method:alignment}, which have unit weights and are averaged over a batch of $N$ frames.
For frame $n$, let $\mathbf{z}_n = E(\mathbf{x}^\text{ras}_n)$ and $\mathbf{z}'_n = E'(\mathbf{x}^\text{cam}_n)$ be the raster and camera latents, each of $D$ values, let $\pi_n = \pi(\cdot \mid \mathbf{x}^\text{ras}_n, \mathbf{s}_n)$ and $\pi'_n = \pi_\text{cam}(\cdot \mid \mathbf{x}^\text{cam}_n, \mathbf{s}_n)$ be the action distributions of the two policies, and let $V$ be the value head of $H$.
The losses are
{\allowdisplaybreaks%
\begin{gather}%
  \mathcal{L}_\text{lat} = \frac{1}{N D\,\sigma_z^2} \sum_{n=1}^{N} \big\|\mathbf{z}'_n - \mathbf{z}_n\big\|_2^2, \\
  \mathcal{L}_\text{KL} = \frac{1}{N} \sum_{n=1}^{N} \mathrm{KL}\big(\pi_n \,\big\|\, \pi'_n\big), \\
  \mathcal{L}_V = \frac{1}{N} \sum_{n=1}^{N} \ell_1^\mathrm{smooth}\Big(\frac{V(\mathbf{z}'_n, \mathbf{s}_n) - V(\mathbf{z}_n, \mathbf{s}_n)}{\sigma_V}\Big),
\end{gather}}%
where $\sigma_z^2$ is the variance of the raster latents and $\sigma_V$ the standard deviation of the value of \argusraster, both measured on the alignment data before training, and $\ell_1^\mathrm{smooth}$ is the smooth L1 loss with threshold 1.
The action loss is this forward KL, at temperature 1.

\paragraph{Training.}
\argus is aligned from \argusraster extended to logged traffic and trained with the ego hood, while the rasterizer renders the twins, \argusraster runs online at every step, and the camera images are decoded on the fly, so that the alignment stores no latents.
It runs for 20 epochs in about 6\,h on 8 H100 GPUs, 48 H100 GPU-hours, the last adapter is kept so that no benchmark scene chooses the checkpoint, and \autoref{tab:align_hparams}c gives its hyperparameters.



==> sec/B_protocol.tex <==
\section{Experimental protocol}
\label{sec:protocol}

Apart from the self-play comparison with \alberti on the CARLA maps (\autoref{tab:selfplay_pictura}), the results of \autoref{sec:exp} come from driving in closed loop on four benchmarks, AlpaSim~\cite{nvidia2025alpasim}, NavSafe-$\infty$~\cite{bao2026navsafe}, Odyssey~\cite{kim2026odyssey}, and HUGSIM~\cite{zhou2026hugsim}; \autoref{sec:protocol:benchmarks} describes each benchmark and its metrics.
\autoref{sec:protocol:compare} gives how our policies run on them and the sources of the results.

\subsection{Benchmarks and metrics}
\label{sec:protocol:benchmarks}

\paragraph{AlpaSim.}
AlpaSim's 2026 challenge~\cite{nvidia2025alpasim} has two tracks, PAI and nuPlan.

\emph{Scenes and scoring.}
AlpaSim replays reconstructed real scenes, of about 20\,s on the PAI track and about 5.5\,s on the nuPlan track.
The PAI track uses NuRec reconstructions of real drives and releases training and validation scenes but no test scenes, so results on it, ours as those of OPTED~\cite{dacol2026opted} and the other works that report on it, are on its 441 validation scenes, the PAI validation scenes.
The nuPlan track uses the WorldEngine~\cite{li2026worldengine} reconstructions of the 1{,}485 scenes of NAVSIM navtest~\cite{dauner2024navsim}.
Its neural reconstructions are faithful only near the path along which each scene was recorded, so AlpaSim restricts the drive to a corridor of 4\,m on each side of that path.
A scene fails after an at-fault collision, an off-road event, or an exit from this corridor, and a failed scene scores 0.
A completed scene with route progress $p$ scores $\min(p/0.8,\,1)$, so a score of 1 means a scene completed over at least 80\% of its route.
A later fix of the scorer (commit \texttt{1b024f0}), the corridor fix, fails a scene only on a sideways exit from the corridor.

\emph{Driver.}
AlpaSim calls the driver of a policy at 10\,Hz and moves the ego with its own controller, which tracks the plan that the driver returns; on the nuPlan track, a new plan is expected every 0.5\,s, the cadence of the track, and on the PAI track, the challenge renders AlpaSim's ego hood on the front camera by default.

\emph{Route and traffic.}
At every call, AlpaSim sends the driver the HD map of the scene and a route, but no speed limit.
AlpaSim builds the route by projecting the recorded drive onto the centers of its lanes and then continuing it along the lanes.
The other road users replay the log, and the drive starts from AlpaSim's state at the end of a warm-up of 1.7\,s on the log.

\paragraph{NavSafe-$\infty$.}
NavSafe-$\infty$~\cite{bao2026navsafe} gathers 280 safety-critical scenarios and scores a policy by its driving score and success rate.
Every policy receives the same inputs, the camera images, the ego state, the driving command, and the next waypoint, without any map or other road users, and plans again every 0.5\,s; the scores are the mean over three evaluation seeds.

\paragraph{Odyssey.}
Odyssey~\cite{kim2026odyssey} scores a policy by its route driving score on 100 scenes, in non-reactive and in reactive traffic, with the route of its standard-definition map.

\paragraph{HUGSIM.}
\label{sec:protocol:hugsim}
\input{tab/hugsim_protocols}
Results on HUGSIM~\cite{zhou2026hugsim} are reported under the three protocols of \autoref{tab:hugsim_protocols}.
The official HD-Score scores the plan that a policy returns at each step.
The realized HD-Score, which TerraTransfer~\cite{xiong2026terratransfer} calls the closed-loop HD-Score, scores the path that the ego drives, so it also applies to policies that output actions.
Only under the protocol of TerraTransfer (\autoref{tab:hugsim_published}b) does it take route completion along the track, as TerraTransfer does.
The pre-challenge protocol is the setting of earlier results, and the protocol of TerraTransfer runs at 10\,Hz.

\subsection{Evaluation setup and comparisons}
\label{sec:protocol:compare}

\paragraph{Our runs.}
\label{sec:protocol:ours}
By default, our policies drive with their trajectory head.
Being reactive, they need not run at their training step: the self-play policy trains at 0.3\,s and the extension at 0.1\,s, but in evaluation each policy decides at every call of the simulator, from the current state, and a jerk action is integrated over the step of the simulator, as Gigaflow also raises its control frequency for evaluation~\cite{cusumanotowner2025gigaflow}.
Our rows and the linear-MPC baselines run through the same driver with AlpaSim's linear MPC, scored after the corridor fix, and on the PAI track with AlpaSim's ego hood, as in the challenge; on the nuPlan track, the trajectory head plans every 0.5\,s.
\argusraster rasterizes the HD map of the scene into its raster views, while \argus reads only the camera images; both place their three goals 40, 60, and 80\,m ahead along AlpaSim's route and are given a speed limit of 40\,m/s, inside their training range.
On Odyssey, \argus plans every 0.1\,s and places its three goals at the same distances along the route that the benchmark gives.
On NavSafe-$\infty$, it plans every 0.5\,s from the inputs given to every policy, which include no route.
Its goals therefore lie on a simple route built from the next waypoint and the driving command: the route passes through the waypoint, then continues straight, or turns by 90$^\circ$ with a radius of 15\,m if the command is left or right.
On HUGSIM, every policy has access to the route of the scenario, which HUGSIM provides together with a turn command derived from it.
The planner baselines are built to take this command, and \argusraster and \argus, which drive toward goals, take three waypoints up to 120\,m ahead on the same route.
The 10\,Hz protocol of TerraTransfer matches the 0.1\,s step of our policies.

\paragraph{Sources of the numbers.}
On AlpaSim, each baseline is reported on each track with the better of two controllers:
\begin{itemize}[leftmargin=*,noitemsep,topsep=2pt]
  \item AlpaSim's nonlinear MPC, taken from the results of \texttt{py123d\_garage}~\cite{kesai2026py123dgarage}, which run three rollouts at AlpaSim commit \texttt{e121e59} (a commit that includes the corridor fix) and whose scores are marked $\dagger$.
  \item AlpaSim's linear MPC, which we run as our runs with one rollout per scene and, as in the challenge, with AlpaSim's ego hood on the front camera on the PAI track.
\end{itemize}
On AlpaSim, LTF, DiffusionDrive, and GTRS-Dense are run only from the checkpoints that SimScale~\cite{tian2026simscale} releases, trained with its synthetic data and marked \simscale{}, while DrivoR is run both with and without them.
\autoref{tab:alpasim} marks the results that OPTED~\cite{dacol2026opted} reports on the PAI track, because they use the scorer from before the corridor fix.
On NavSafe-$\infty$ and Odyssey (\autoref{tab:alpasim}b and c, \autoref{tab:navsafe_odyssey}), the baselines are the published numbers that \texttt{py123d\_garage}~\cite{kesai2026py123dgarage} gathers, and DrivoR \simscale{} and \argus are our runs.
On HUGSIM, every row of \autoref{tab:hugsim}a and of \cref{tab:hugsim_4hz,tab:hugsim_10hz} is our run of the released checkpoint, except for ECO~\cite{zhang2026eco}, whose code is not released and which is run from our reimplementation.
Under the published protocols (\autoref{tab:hugsim}b and c, \autoref{tab:hugsim_published}), the baselines are the numbers reported by Gigapixel~\cite{rowe2026gigapixel} and DriveZero~\cite{he2026drivezero}, and by TerraTransfer~\cite{xiong2026terratransfer}.

\paragraph{Which rows are compared.}
Only camera policies are ranked against each other.
\cref{tab:alpasim,tab:hugsim} compare \argus with the camera planners.
The tables of the appendix add policies that do not read camera images, without ranking them: \argusraster with its trajectory head in \cref{tab:alpasim_all,tab:hugsim_4hz,tab:hugsim_10hz,tab:hugsim_published} and with its action head in \cref{tab:hugsim_4hz,tab:hugsim_10hz}, the vectorized policy in \cref{tab:hugsim_4hz,tab:hugsim_10hz}, and a constant-velocity baseline in \autoref{tab:alpasim_all}.
In the main paper, \autoref{tab:pipeline} follows \argusraster from self-play to its trajectory head, with the best camera planner for reference, and \autoref{fig:policy_swap} gives the share of the score of \argusraster and of the vectorized policy that the camera policy aligned from each keeps.

\paragraph{The vectorized policy.}
The privileged policy of the policy swap in \autoref{sec:exp:vectorized} drives from the state of the scene itself, given in the ego frame as lists of map elements, agents, and traffic lights.
Unlike the raster views, these lists are not limited to what the cameras see: the agent list holds the agents closest to the ego within 100\,m, occluded or not, each with its exact speed and its velocity relative to the ego.
The policy thus relies on information that camera images do not give, which is why the camera policy aligned to it keeps less of its driving (\autoref{sec:exp:vectorized}).
Like the vectorized policies of Gigaflow~\cite{cusumanotowner2025gigaflow} and PufferDrive~\cite{cornelisse2025pufferdrive}, it has its own architecture, which encodes each list with a small network instead of reading images; only its outputs are those of \argusraster, the same 12 jerk actions and a value.

\emph{Inputs.}
The map lists hold up to 70 lane segments, every second one along each lane, and 50 road-edge segments, all taken from the same corridor as the raster views and each described by its position, half-length, and heading.
The agent list holds up to 20 agents within 100\,m of the ego, each described by its position, size, and heading, by its own speed, and by its velocity relative to the ego, in two components.
The traffic-light list holds up to 4 traffic lights within 100\,m of the ego, each described by the positions of the two ends of its stop line, the height of the line, and the state of the light.

\emph{Network.}
Mirroring the choices of Gigaflow~\cite{cusumanotowner2025gigaflow} and PufferDrive~\cite{cornelisse2025pufferdrive}, each element passes through a two-layer MLP with LayerNorm, and each list is then max-pooled over its elements.
An MLP trunk of three layers of width 1024 with GELU maps the four pooled lists, the ego state, and the conditioning vector to the 12 jerk actions and the value, and, as in \argusraster, the actor and the critic share the whole network.

\emph{Training and alignment.}
The policy is trained in self-play and extended to logged traffic with the same RL recipe as \argusraster (see \autoref{sec:impl:selfplay} and \autoref{sec:impl:logged}).
After the training extension, it reaches 9.99 goals per vehicle in self-play on the CARLA maps with 50 agents per scene, against 13.87 for \argusraster after the same extension, w/~action, at the same density, and its at-fault vehicle collision rate is 0.088 against 0.065; \autoref{tab:selfplay_pictura} instead scores the self-play policy, before the extension, at the medium density of \pictura.
An image encoder is then aligned to it with the same three losses and data as \argus.
$\mathcal{L}_\text{KL}$ and $\mathcal{L}_V$ are unchanged, and $\mathcal{L}_\text{lat}$ regresses the output of the image encoder onto the scene latents of the policy, which take another form: the 896 values of its four pooled lists, the input that its trunk reads besides the ego state and the conditioning.
The image encoder thus takes the place of the list encoders and feeds the frozen trunk, the connection to the policy that TerraTransfer~\cite{xiong2026terratransfer} also uses.
To produce these 896 values, the image encoder keeps the backbone and adapter of \argus, which give 16 tokens of width 128 per camera, but has no copy of the scene pooler, since the policy has none: the max-pooling over its lists plays that role, and a pooler of 32 learned latents maps the tokens to the 896 values in its place.


==> sec/C_results.tex <==
\section{Additional results}
\label{sec:more_results}

This section details the experiments of \autoref{sec:exp}.
\autoref{sec:more_results:compare} gives the detailed comparison with camera planners, and \autoref{sec:more_results:qualitative} presents qualitative results and where \argus fails against \argusraster.
\autoref{sec:more_results:selfplay} evaluates \argusraster in self-play, against \alberti and along its training, and \autoref{sec:more_results:ablation} gives the protocol and detailed results of each ablation.

\subsection{Comparison with camera planners}
\label{sec:more_results:compare}

Tabs.~\ref{tab:alpasim_all} to~\ref{tab:navsafe_odyssey}, which detail the comparison with camera planners, are grouped at the end of the appendix.

\paragraph{AlpaSim.}
\autoref{tab:alpasim_all} completes \autoref{tab:alpasim}a with the failure rates of each track.
On the PAI track, only DrivoR has a lower collision or off-road rate than \argus, but it covers only 53.2\% of the route, and 41.8\% with SimScale, against 90.6\% for \argus.
Per distance driven, \argus is the safer policy: it drives 1.90\,km per at-fault collision or off-road event, against 0.68\,km for DrivoR and 0.91\,km with SimScale.
TransFuser-K1 exits the corridor least often on both tracks.
The corridor, 4\,m on each side of the recorded path, bounds where the reconstructions stay faithful, so this rate also counts drives that depart from the logged path.

\paragraph{NavSafe-$\infty$ and Odyssey.}
Tabs.~\ref{tab:alpasim}b and \ref{tab:alpasim}c are completed by \autoref{tab:navsafe_odyssey}, with the scores behind the plots and the number of parameters of each planner.

\paragraph{HUGSIM.}
In the default protocol of HUGSIM, the first of the three that \autoref{tab:hugsim_protocols} lists, \autoref{tab:hugsim_4hz} completes \autoref{tab:hugsim}a with every policy we run, with either head, and both scores by difficulty.
In the pre-challenge and TerraTransfer protocols, panels (a) and (b) of \autoref{tab:hugsim_published} complete \autoref{tab:hugsim}b and c with the score by difficulty.
Finally, \autoref{tab:hugsim_10hz} scores the policies of \autoref{tab:hugsim_4hz} on all 436 scenarios at the 10\,Hz step of TerraTransfer~\cite{xiong2026terratransfer}.
In its own protocol, panel (b) of \autoref{tab:hugsim_published}, TerraTransfer computes the realized HD-Score with route completion measured along the track: the farthest distance that the ego reaches along the recorded camera track, as a fraction of the length of the track.
\autoref{tab:hugsim_10hz} instead uses the route completion of HUGSIM's own HD-Score, which keeps it closer to the original benchmark; its scores thus differ from those of panel (b).

\subsection{Qualitative results}
\label{sec:more_results:qualitative}
\input{tab/failures}
The project page, \projectpage, shows qualitative results.
This section summarizes what the page shows and where \argus fails against \argusraster.

\paragraph{Qualitative results.}
It shows closed-loop drives of \argus in AlpaSim on PAI validation scenes, each from the five cameras that \argus reads, with the trajectory that it plans drawn on the front one.
Six drives pass: a roundabout, a narrow street, a commercial street with a turn, a night scene where \argus yields to a pedestrian, slowing almost to a stop, a hillside road, and a motorway at 122\,km/h.
Three drives fail, and the next paragraph describes them.

\paragraph{Failures.}
On the PAI track, \argus scores 4.6 points below \argusraster, the policy it is aligned from, and \autoref{tab:failures} counts the failed scenes of both.
Most of the gap comes from leaving the road, in 23 scenes against 3, while collisions stay close, in 23 scenes against 18.
The off-road events tend to happen where the logged drive passes close to the curb: the smallest distance of the logged car to the curb separates the 17 scenes in which \argus leaves the road and \argusraster passes from the 360 scenes that both pass with an AUC of 0.90.
The linked page shows two of them: \argus leaves the road in snow, and clips the road edge in a narrow street.
The curb can be ambiguous in the camera images of \argus, whereas it never is in the raster views of \argusraster, which draw it from the map.
Exits from the corridor are as frequent for both policies, 19 scenes each, and make up 19 of the 65 failures of \argus and 19 of the 40 of \argusraster.
Such an exit does not necessarily mean unsafe driving: in the third failure of the linked page, \argus leaves the corridor but finishes without any collision or off-road event.
On the nuPlan track, the two policies are on par, at 95.9 and 95.8.

\subsection{Self-play of \argusraster}%
\label{sec:more_results:selfplay}
This section studies the self-play policy, \argusraster after self-play only and driving with its action head, the ``Self-play, w/~action'' row of \autoref{tab:pipeline}: it compares it with \alberti, follows its score along self-play, and measures what single-agent PPO on logged scenes adds.

\paragraph{Against \alberti.}

\autoref{tab:selfplay_pictura} compares the self-play policy with the published numbers of \alberti~\cite{yin2026pictura}, under the self-play protocol of \pictura on the CARLA maps.
The self-play policy is more cautious: it reaches fewer goals, 8.68 per agent against 11.21, but has better safety metrics, with 105.9\,km per infraction against 11.6.
\input{tab/selfplay_pictura}%

\paragraph{Scaling self-play.}
\autoref{fig:selfplay_scaling} shows how the score of the self-play policy evolves along self-play.
The score rises from 25.2 to 57.4 by about 40B steps, and reaches 61.1 at the end of self-play, after the learning-rate decay.
\input{fig/selfplay_scaling}%

\input{fig/data_source}%
\input{fig/backbone_analysis}%
\paragraph{Single-agent PPO.}
Single-agent PPO is the extension of self-play to logged scenes (\autoref{sec:impl:logged}).
On the PAI track, this raises its score from 61.1 to 89.3 (\autoref{tab:selfplay_extension_pai}), and most of the gain comes from scenes where the self-play policy is rear-ended, which drop from 147 to 13.
In AlpaSim, a rear-end does not count as a failure, but it cuts the progress of the drive.
After this extension, \argusraster passes 134 of these 147 scenes, and its higher progress on them accounts for about two thirds of the gain.
These rear-ends are an artifact of log-replay evaluation: the logged cars do not react to an ego that drives slower than the logged one, whereas in self-play the traffic is reactive.

\input{tab/selfplay_extension_pai}%

\subsection{Ablations}
\label{sec:more_results:ablation}

\subsubsection{Alignment data}%
\label{sec:ablation:data}

\paragraph{Collection method.}
The main paper aligns \argus on frames of the drives of \argusraster in AlpaSim that score 1.
\autoref{fig:data_source} compares this default with three other collections, for the same number of steps: the logged human drives, all the drives of \argusraster including failures, and both human drives and drives of \argusraster.
In every collection, the logged human drives included, the frames are rendered in reconstructed scenes, by NuRec for PAI and WorldEngine for navtrain.
All of them score close to the default, within 0.5 point on PAI and 0.6 on nuPlan.

\subsubsection{Alignment design}
\label{sec:ablation:alignment}

This section ablates two design choices of the alignment: its losses and its image backbone.

\paragraph{Losses.}
\autoref{tab:alignment_losses}b removes each of the three losses of \autoref{sec:method:alignment} in turn, and also keeps the latent loss $\mathcal{L}_\text{lat}$ alone, each with three seeds.
The seeds spread little, by at most 1.5 points, for every setting but one: without $\mathcal{L}_\text{lat}$, the mean score drops by 16 points on PAI and 12 on HUGSIM, and the seeds spread by $\pm 5.0$ and $\pm 4.4$.
$\mathcal{L}_\text{lat}$ alone is on par with $\mathcal{L}_\text{\argus}$ on PAI, 84.0 against 84.2, and ahead on HUGSIM, 59.1 against 56.7.
Removing $\mathcal{L}_V$ moves every score by at most 0.6 point, within the spread of the seeds.


\paragraph{Image backbone.}
\autoref{fig:backbone_analysis} aligns \argus with other image backbones, with the same recipe otherwise.
\argus does not depend on DINOv3, and the DINO families work best.
DINOv2 ViT-B/14~\cite{oquab2024dinov2}, the backbone of \argusplus, gives our best score on PAI, 87.3 against 84.2 for the default DINOv3 ViT-S/16, and nearly our best on nuPlan, 96.1, which shows room for improvement beyond our default DINOv3 ViT-S/16.
Small backbones work surprisingly well: three towers of about 5.5M parameters lose only 0.2 to 0.4 point to the default on nuPlan, and their 80.0 to 82.2 on PAI still lead every camera planner of \autoref{tab:alpasim}a.
These towers are EUPE-T/16~\cite{zhu2026eupe}, PE-T/16~\cite{bolya2025perceptionencoder}, and a ViT-T/16 that Lightly\footnote{LightlyTrain 0.18.0, \url{https://docs.lightly.ai/train/stable/pretrain_distill/models/dinov3.html}.} distills from DINOv3 ViT-L/16.
Encoders trained for other tasks, Depth Anything V2-S~\cite{yang2024depthanythingv2} (depth), SigLIP~2 ViT-B/16~\cite{tschannen2025siglip2} (vision and language), and SAM ViT-B/16~\cite{kirillov2023sam} (segmentation), score 82.8 to 83.6 on PAI, below the DINO backbones of their size.
\autoref{tab:backbone_gpuh} gives the GPU-hours of each alignment.

\input{tab/backbone_gpuh}

\subsubsection{Trajectory head}%
\label{sec:ablation:traj}
Over the three seeds of \autoref{tab:traj_head}a, the trajectory-head ablation holds.
DAgger gains 2.1 points over behavior cloning on PAI and 1.5 on HUGSIM, while the two are level on nuPlan.
The flow head scores above the MSE and WTA heads on PAI and HUGSIM, while all three are within half a point on nuPlan.

\clearpage
\input{tab/alpasim_navsafe_odyssey_full}%
\input{tab/hugsim_full}%




==> tab/alpasim_all.tex <==
\begin{table*}[tp]
  \centering
  \caption{\textbf{Full closed-loop results on AlpaSim.} \autoref{tab:alpasim} with every metric.
    Score: official AlpaSim metric, route progress capped at 80\%, zero for a failed scene; Coll., Off., Corr.: scenes failed by an at-fault collision, an off-road event, or an exit from the corridor, in percent; Prog.: progress along the logged route, clamped to [0, 1] per scene, in percent; km/inf.: km per at-fault collision or off-road event.
    On each track, each baseline with the better of AlpaSim's linear and nonlinear MPC. Shaded: the score of each track; \textbf{bold}, \underline{underlined}: best, second best among camera policies.}
  \label{tab:alpasim_all}
 
  \scriptsize
  \setlength{\tabcolsep}{3.4pt}
  \sbox0{%
  \begin{tabular}{lr>{\columncolor{keycol}}cccccc>{\columncolor{keycol}}cccccc}
    \toprule
    & & \multicolumn{6}{c}{PAI track} & \multicolumn{6}{c}{nuPlan track} \\
    \cmidrule(lr){3-8} \cmidrule(lr){9-14}
    Method & Params. & Score\,$\uparrow$ & Coll.\,$\downarrow$ & Off.\,$\downarrow$ & Corr.\,$\downarrow$ & Prog.\,$\uparrow$ & km/inf.\,$\uparrow$ & Score\,$\uparrow$ & Coll.\,$\downarrow$ & Off.\,$\downarrow$ & Corr.\,$\downarrow$ & Prog.\,$\uparrow$ & km/inf.\,$\uparrow$ \\
    \midrule
    Constant velocity & -- & 21.7 & 18.6 & 22.7 & 22.9 & 51.1 & 0.27 & 53.1 & 5.1 & 17.0 & 13.2 & 69.6 & 0.11 \\
    \rowcolor{rasterrow} \argusraster & 4.9M & 88.8 & 4.1 & 0.7 & 4.3 & 93.1 & 4.19 & 95.8 & 0.4 & 1.1 & 1.5 & 94.6 & 2.18 \\
    \midrule
    Qwen-Drive 1.0~\cite{zhou2026qwendrive} & 5.1B & 25.4$^{\ddagger}$ & 14.4 & 18.3 & 19.0 & 39.1 & 0.21 & -- & -- & -- & -- & -- & -- \\
    LTFv6~\cite{nguyen2026lead} & 62.1M & 26.5$^{\ddagger}$ & 10.2 & 20.7 & 27.6 & 43.7 & 0.23 & -- & -- & -- & -- & -- & -- \\
    LTFv6 + OPTED~\cite{dacol2026opted} & 62.1M & 41.8$^{\ddagger}$ & 23.4 & 11.7 & 18.6 & 73.4 & 0.43 & -- & -- & -- & -- & -- & -- \\
    Alpamayo 1~\cite{nvidia2025alpamayo} & 10.5B & 56.0$^{\dagger}$ & 5.4 & 10.3 & 24.3 & 75.3 & 0.96 & -- & -- & -- & -- & -- & -- \\
    Alpamayo 1.5~\cite{nvidia2025alpamayo} & 10.5B & 55.3$^{\dagger}$ & 5.2 & 11.3 & 25.4 & 76.3 & 0.94 & -- & -- & -- & -- & -- & -- \\
    LTF \simscale~\cite{chitta2023transfuser,tian2026simscale} & 56.0M & 38.8 & 10.2 & 10.9 & 17.2 & 50.4 & 0.41 & 88.4 & 1.0 & 5.7 & 1.4 & 89.3 & 0.43 \\
    DiffusionDrive \simscale~\cite{liao2025diffusiondrive,tian2026simscale} & 60.8M & 40.3 & 7.0 & 8.6 & 10.0 & 44.6 & 0.49 & 87.8 & 0.7 & 6.0 & 1.7 & 88.8 & 0.43 \\
    GTRS-Dense \simscale~\cite{li2025gtrs,tian2026simscale} & 81.0M & 52.9 & 10.9 & 7.7 & 16.8 & 66.5 & 0.66 & 88.5$^{\dagger}$ & 0.9 & 3.7 & 2.5 & 82.9 & 0.35 \\
    DrivoR~\cite{kirby2026drivor} & 40.8M & 50.4 & 8.4 & \underline{4.8} & 7.9 & 53.2 & 0.68 & 91.0 & 1.2 & 3.5 & 1.8 & 90.9 & 0.63 \\
    DrivoR \simscale~\cite{kirby2026drivor,tian2026simscale} & 40.8M & 42.8 & \underline{3.4} & \underline{4.8} & 6.8 & 41.8 & 0.91 & 90.5 & \textbf{0.4} & 2.3 & 2.0 & 87.9 & 1.06 \\
    TransFuser-K1~\cite{kesai2026py123dgarage} & 67.7M & 78.4$^{\dagger}$ & 7.0 & 5.8 & \textbf{3.3} & 84.6 & 1.44 & 90.3$^{\dagger}$ & \underline{0.5} & 3.3 & \textbf{0.8} & 79.6 & 0.72 \\
    \rowcolor{argusrow} \argus & 31.7M & \underline{84.2} & 5.2 & 5.2 & \underline{4.3} & \underline{90.6} & \underline{1.90} & \underline{95.9} & 0.6 & \underline{1.3} & \underline{1.3} & \underline{94.9} & \underline{1.72} \\
    \rowcolor{argusrow} \argusplus & 98.5M & \textbf{87.3} & \textbf{2.9} & \textbf{4.1} & \underline{4.3} & \textbf{91.9} & \textbf{2.84} & \textbf{96.1} & \textbf{0.4} & \textbf{1.2} & \underline{1.3} & \textbf{95.0} & \textbf{2.00} \\
    \bottomrule
  \end{tabular}
  \unskip}\usebox0\par\vspace{2pt}
  \begin{minipage}{\wd0}\scriptsize\raggedright $^{\dagger}$\,all metrics of that track with the nonlinear MPC, from \texttt{py123d\_garage}~\cite{kesai2026py123dgarage};\enspace$^{\ddagger}$\,as reported by OPTED~\cite{dacol2026opted}, scored before the corridor fix.\par\end{minipage}%
\end{table*}


==> tab/alpasim_navsafe_odyssey_full.tex <==
\begin{table*}[tp]
  \centering
  \begingroup\renewenvironment{table*}[1][]{}{}\input{tab/alpasim_all}\endgroup
  \par\vspace{14pt}
  \begin{minipage}[t]{\textwidth}\centering%
    \begingroup\renewenvironment{table}[1][]{}{}\input{tab/navsafe_odyssey}\endgroup
  \end{minipage}
\end{table*}


==> tab/backbone_gpuh.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{Training cost of the backbones}: A100 GPU-hours of the alignment of \argus with each image backbone of \autoref{fig:backbone_analysis}, on 8 to 32 GPUs.
    Params: parameters of the pretrained checkpoint; $^{\dagger}$: trained on H100, A100-hours estimated as 1.8 times the H100-hours, the ratio measured with DINOv3 ViT-S/16 on both. Shaded: default.}
  \label{tab:backbone_gpuh}
  \scriptsize
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{lrr}
    \toprule
    Model & Params (M) & GPU-h \\
    \midrule
    \rowcolor{argusrow} DINOv3 ViT-S/16 & 21.6 & 86 \\
    DINOv3 ViT-B/16 & 85.7 & $\sim$200$^{\dagger}$ \\
    DINOv2 ViT-S/14 & 22.1 & 125 \\
    DINOv2 ViT-B/14 & 86.6 & 328 \\
    Depth Anything V2-S & 22.1 & 125 \\
    EUPE-T/16 & 5.5 & 51 \\
    PE-T/16 & 5.7 & 51 \\
    ViT-T/16 (Lightly) & 5.5 & 51 \\
    SigLIP~2 ViT-B/16 & 93.5 & 233 \\
    SAM ViT-B/16 & 89.7 & 652 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tab/failures.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{Failures on the PAI track}: AlpaSim scene score and failed scenes of \argus and \argusraster out of the 441 PAI validation scenes, each counted once, under the first cause in the order at-fault collision, off-road, corridor exit.}
  \label{tab:failures}
  \scriptsize
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{lrrrrr}%
    \toprule
    & Score & Collision & Off-road & Corridor exit & All \\
    \midrule
    \argus & 84.2 & 23 & 23 & 19 & 65 \\
    \argusraster & 88.8 & 18 & 3 & 19 & 40 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tab/hugsim_10hz.tex <==
\begin{table}[tp]
  \centering
  \caption{\textbf{Full closed-loop results on HUGSIM in the non-default 10\,Hz setting.}
    \autoref{tab:hugsim_4hz} at 10\,Hz, the rate of TerraTransfer~\cite{xiong2026terratransfer}: HD-Score and realized HD-Score over the 436 scenarios; \textbf{bold}, \underline{underlined}: best, second best among camera policies.}
  \label{tab:hugsim_10hz}
  \footnotesize
  \setlength{\tabcolsep}{3pt}
  \sbox0{%
  \begin{tabular}{lrcc}
    \toprule
    Method & Params. & HD-Score $\uparrow$ & \begin{tabular}[b]{@{}c@{}}Realized\\HD-Score $\uparrow$\end{tabular} \\%
    \midrule
    \rowcolor{vecrow} \vectorized & 3.8M & -- & 71.9 \\
    \rowcolor{rasterrow} Self-play, w/~action & 2.9M & -- & 75.7 \\
    \rowcolor{rasterrow} \argusraster & 4.9M & 69.1 & 71.8 \\
    \rowcolor{rasterrow} \actrow & 2.9M & -- & 71.2 \\
    \midrule
      UniAD~\cite{hu2023uniad} & 131.8M & 37.0 & 46.0 \\
      VAD~\cite{jiang2023vad} & 58.4M & 18.2 & 23.1 \\
      LTF~\cite{chitta2023transfuser} & 56.0M & 28.2 & 36.0 \\
      LTFv6~\cite{nguyen2026lead} & 62.1M & 46.0 & 51.3 \\
      GTRS-Dense~\cite{li2025gtrs} & 81.0M & 46.1 & 50.1 \\
      GTRS-Aug~\cite{li2025gtrs} & 86.4M & 42.7 & 44.4 \\
      DrivoR~\cite{kirby2026drivor} & 40.8M & 45.9 & 47.7 \\
      DrivoR + ECO$^{*}$~\cite{zhang2026eco} & 40.8M & \underline{48.0} & 49.3 \\
      TOAD~\cite{xu2026toad} & 40.8M & 47.6 & 49.8 \\
      ZTRS~\cite{li2025ztrs} & 83.4M & 46.9 & 48.1 \\
      VaVAM-B~\cite{bartoccioni2025vavam} & 357.3M & 17.4 & 34.6 \\
      VaVAM-B + ECO$^{*}$~\cite{zhang2026eco} & 357.3M & 37.1 & 40.5 \\
    \rowcolor{argusrow} \argus & 31.7M & \textbf{67.0} & \textbf{69.6} \\
    \rowcolor{argusrow} \actrow & 29.7M & -- & \underline{65.6} \\
    \bottomrule
  \end{tabular}
  \unskip}\usebox0\par\vspace{2pt}
  \begin{minipage}{\wd0}\scriptsize\raggedright $^{*}$\,our reimplementation.\par\end{minipage}
\end{table}



==> tab/hugsim_4hz.tex <==
\begin{table*}[tp]
  \centering
  \caption{\textbf{Full closed-loop results on HUGSIM in its default setting.}
    \autoref{tab:hugsim} with every policy we run and the score by difficulty (easy, medium, hard, extreme); per-dataset scores in \autoref{tab:hugsim}; shaded: the score over all scenarios; \textbf{bold}, \underline{underlined}: best, second best among camera policies.}
  \label{tab:hugsim_4hz}
  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \sbox0{%
  \begin{tabular}{lr>{\columncolor{keycol}}ccccc<{\hspace{6pt}}>{\columncolor{keycol}}ccccc}%
    \toprule
    & & \multicolumn{5}{c}{HD-Score $\uparrow$} & \multicolumn{5}{c}{Realized HD-Score $\uparrow$} \\
    \cmidrule(lr){3-7} \cmidrule(l){8-12}
    Method & Params. & All & Easy & Med. & Hard & Ext. & All & Easy & Med. & Hard & Ext. \\
    \midrule
    \rowcolor{vecrow} \vectorized & 3.8M & -- & -- & -- & -- & -- & 60.8 & 85.7 & 71.7 & 46.7 & 38.2 \\
    \rowcolor{rasterrow} \argusraster & 4.9M & 54.5 & 87.3 & 61.9 & 42.5 & 29.1 & 58.4 & 87.4 & 66.6 & 47.0 & 33.9 \\
    \rowcolor{rasterrow} \actrow & 2.9M & -- & -- & -- & -- & -- & 60.9 & 88.1 & 67.5 & 51.0 & 39.1 \\
    \midrule
     UniAD~\cite{hu2023uniad} & 131.8M & 29.8 & 59.2 & 36.5 & 18.9 & 6.7 & 39.4 & 71.4 & 47.5 & 27.3 & 13.5 \\
     VAD~\cite{jiang2023vad} & 58.4M & 12.4 & 34.8 & 7.9 & 7.2 & 6.5 & 23.3 & 43.8 & 21.5 & 18.6 & 14.3 \\
     LTF~\cite{chitta2023transfuser} & 56.0M & 20.9 & 55.0 & 15.9 & 9.6 & 12.8 & 30.6 & 60.3 & 27.6 & 19.8 & 22.2 \\
     LTFv6~\cite{nguyen2026lead} & 62.1M & 34.9 & 74.4 & \underline{44.9} & 16.9 & 5.8 & 41.3 & 77.7 & 51.4 & 24.9 & 13.1 \\
     GTRS-Dense~\cite{li2025gtrs} & 81.0M & 34.4 & 75.6 & 37.6 & 18.3 & 12.5 & 41.1 & 76.8 & 46.3 & 25.5 & 19.8 \\
     GTRS-Aug~\cite{li2025gtrs} & 86.4M & 28.9 & 74.8 & 24.8 & 12.6 & 14.7 & 36.1 & 73.2 & 35.5 & 21.6 & 21.8 \\
     DrivoR~\cite{kirby2026drivor} & 40.8M & 33.5 & 76.1 & 33.3 & 16.2 & \underline{16.7} & 40.1 & 73.5 & 43.3 & 24.6 & 23.6 \\
     DrivoR + ECO$^{*}$~\cite{zhang2026eco} & 40.8M & 32.9 & 77.0 & 32.7 & 14.4 & 16.1 & 39.2 & 73.2 & 42.5 & 22.6 & 23.3 \\
     TOAD~\cite{xu2026toad} & 40.8M & \underline{36.1} & 75.9 & 41.1 & 16.9 & 15.3 & 41.8 & 75.3 & 48.1 & 24.4 & 22.3 \\
     ZTRS~\cite{li2025ztrs} & 83.4M & 34.9 & \underline{77.4} & 35.0 & \underline{21.4} & 14.3 & 42.0 & 76.9 & 45.3 & 29.5 & 21.4 \\
     VaVAM-B~\cite{bartoccioni2025vavam} & 357.3M & 13.4 & 26.8 & 16.0 & 7.5 & 4.4 & 29.3 & 48.4 & 35.7 & 20.0 & 13.4 \\
     VaVAM-B + ECO$^{*}$~\cite{zhang2026eco} & 357.3M & 25.2 & 45.4 & 29.4 & 17.0 & 10.7 & 32.2 & 51.0 & 37.5 & 23.8 & 17.5 \\
    \rowcolor{argusrow} \argus & 31.7M & \textbf{53.6} & \textbf{85.7} & \textbf{65.8} & \textbf{36.6} & \textbf{25.7} & \textbf{57.4} & \underline{86.5} & \textbf{69.8} & \underline{41.7} & \textbf{30.7} \\
    \rowcolor{argusrow} \actrow & 29.7M & -- & -- & -- & -- & -- & \underline{55.6} & \textbf{88.2} & \underline{64.4} & \textbf{44.0} & \underline{27.7} \\
    \bottomrule
  \end{tabular}
  \unskip}\usebox0\par\vspace{2pt}
  \begin{minipage}{\wd0}\scriptsize\raggedright $^{*}$\,our reimplementation.\par\end{minipage}%
\end{table*}


==> tab/hugsim_full.tex <==
\begin{table*}[tp]
  \centering
  \begingroup\renewenvironment{table*}[1][]{}{}\input{tab/hugsim_4hz}\endgroup
  \par\vspace{12pt}
  \begin{minipage}[t]{0.48\textwidth}\vspace{0pt}\centering
    \begingroup\renewenvironment{table}[1][]{}{}\input{tab/hugsim_10hz}\endgroup
  \end{minipage}\hfill
  \edef\hpanelw{\the\dimexpr0.49\textwidth\relax}%
  \begin{minipage}[t]{0.49\textwidth}\vspace{0pt}\centering
    \begingroup\renewenvironment{table*}[1][]{}{}\input{tab/hugsim_published}\endgroup
  \end{minipage}
\end{table*}


==> tab/hugsim_protocols.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{HUGSIM protocols}: the scenarios, simulator step, and score of each protocol, the published results that use it, and the tables that report our results in it.}
  \label{tab:hugsim_protocols}
  \scriptsize
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{@{}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{2.15cm}>{\raggedright\arraybackslash}p{2.15cm}>{\raggedright\arraybackslash}p{2.15cm}@{}}
    \toprule
    & Default & Pre-challenge & TerraTransfer \\
    \midrule
    Scenarios & 436, current release & 345, pre-challenge release (\texttt{fb8ecd4}) & 88 of the current release, from nuScenes \\
    Step & 0.25\,s (4\,Hz), HUGSIM's default & 0.25\,s (4\,Hz) & 0.1\,s (10\,Hz) \\
    Score & official and realized HD-Score & official HD-Score & realized HD-Score, called closed-loop HD-Score there \\%
    Used by & most published results & Gigapixel, DriveZero & TerraTransfer \\
    Our results & \autoref{tab:hugsim}a, \autoref{tab:hugsim_4hz} & \autoref{tab:hugsim}b, \autoref{tab:hugsim_published}a & \autoref{tab:hugsim}c, \autoref{tab:hugsim_published}b; all 436 scenarios in \autoref{tab:hugsim_10hz} \\
    \bottomrule
  \end{tabular}
\end{table}


==> tab/hugsim_published.tex <==
\begin{table*}[tp]
  \centering
  \caption{\textbf{HUGSIM under published protocols, per difficulty.} The protocols of \autoref{tab:hugsim_bc}b and c.
    Shaded: the score over all scenarios; \textbf{bold}, \underline{underlined}: best, second best among camera policies.}
  \label{tab:hugsim_published}
  \scriptsize
  \setlength{\tabcolsep}{2.6pt}
  \begin{minipage}[t]{\ifdefined\hpanelw\hpanelw\else0.49\textwidth\fi}\vspace{0pt}\centering
    {\bfseries (a) Pre-challenge set, 345 scenarios, official HD-Score}\par
    {\scriptsize as in Gigapixel and DriveZero}\par\vspace{2pt}
  \sbox0{%
  \begin{tabular}{lcccc>{\columncolor{keycol}}c}
    \toprule
    & \multicolumn{5}{c}{HD-Score $\uparrow$} \\
    \cmidrule(lr){2-6}
    Method & Easy & Med. & Hard & Ext. & All \\
    \midrule
    \rowcolor{rasterrow} \argusraster & 81.4 & 62.6 & 43.7 & 40.4 & 55.2 \\
    \midrule
    LTF$^{\S}$~\cite{chitta2023transfuser} & 58.9 & 18.0 & 9.8 & 25.9 & 23.7 \\
    VAD$^{\S}$~\cite{jiang2023vad} & 36.3 & 9.5 & 8.0 & 11.5 & 13.4 \\
    UniAD$^{\S}$~\cite{hu2023uniad} & 64.9 & 45.8 & 20.6 & 6.6 & 32.7 \\
    DrivoR$^{\S}$~\cite{kirby2026drivor} & 73.3 & 34.6 & 18.8 & \underline{32.5} & 35.7 \\
    DrivoR \simscale$^{\S}$~\cite{kirby2026drivor,tian2026simscale} & 64.8 & 50.3 & 16.8 & 25.8 & 38.1 \\
    Gigapixel$^{\S}$~\cite{rowe2026gigapixel} & 67.4 & 51.9 & 19.1 & 21.6 & 38.5 \\
    DriveZero$^{\S}$~\cite{he2026drivezero} & 78.5 & 47.2 & 16.0 & 28.7 & 39.4 \\
    DriveZero-Scale$^{\S}$~\cite{he2026drivezero} & \textbf{81.9} & \underline{60.5} & \underline{24.7} & 27.6 & \underline{46.6} \\
    \rowcolor{argusrow} \argus & \underline{80.4} & \textbf{65.1} & \textbf{37.9} & \textbf{38.9} & \textbf{54.1} \\
    \bottomrule
  \end{tabular}\unskip}\usebox0\par\vspace{2pt}
    \begin{minipage}{\wd0}\scriptsize\raggedright $^{\S}$\,as reported by Gigapixel~\cite{rowe2026gigapixel} and DriveZero~\cite{he2026drivezero}.\par\end{minipage}%
  \end{minipage}\ifdefined\hpanelw\par\vspace{8pt}\else\hfill\fi%
  \begin{minipage}[t]{\ifdefined\hpanelw\hpanelw\else0.49\textwidth\fi}\vspace{0pt}\centering
    {\bfseries (b) nuScenes-10\,Hz, 88 scenarios, realized HD-Score}\par
    {\scriptsize as in TerraTransfer}\par\vspace{2pt}
  \sbox2{%
  \begin{tabular}{lcccc>{\columncolor{keycol}}c}
    \toprule
    & \multicolumn{5}{c}{Realized HD-Score $\uparrow$} \\
    \cmidrule(lr){2-6}
    Method & Easy & Med. & Hard & Ext. & All \\
    \midrule
    \rowcolor{rasterrow} \argusraster & 83.7 & 54.0 & 70.0 & 73.6 & 67.4 \\
    \midrule
    UniAD$^{\S}$~\cite{hu2023uniad} & 36.7 & 19.8 & 24.9 & 10.9 & 22.4 \\
    VAD$^{\S}$~\cite{jiang2023vad} & 40.0 & 22.8 & 24.2 & 9.5 & 23.9 \\
    LTF$^{\S}$~\cite{chitta2023transfuser} & 63.4 & 39.1 & 28.9 & 9.8 & 36.0 \\
    ECO$^{\S}$~\cite{zhang2026eco} & 76.4 & 41.6 & 40.5 & \underline{25.5} & 45.2 \\
    TerraTransfer$^{\S}$~\cite{xiong2026terratransfer} & \underline{76.9} & \textbf{50.1} & \underline{56.0} & 15.0 & \underline{49.0} \\
    \rowcolor{argusrow} \argus & \textbf{82.6} & \underline{49.8} & \textbf{59.2} & \textbf{67.9} & \textbf{62.1} \\
    \bottomrule
  \end{tabular}\unskip}\usebox2\par\vspace{2pt}
    \begin{minipage}{\wd2}\scriptsize\raggedright $^{\S}$\,as reported by TerraTransfer~\cite{xiong2026terratransfer}.\par\end{minipage}%
  \end{minipage}
\end{table*}


==> tab/navsafe_odyssey.tex <==
\begin{table}[tp]
  \centering
  \caption{\textbf{Closed-loop results on NavSafe-$\infty$ and Odyssey.}
    NavSafe-$\infty$: driving score (DS) and success rate (SR, \%), 280 scenarios; Odyssey: route driving score, non-reactive (NR) and reactive (R), 100 scenes.
    \textbf{bold}, \underline{underlined}: best, second best.}
  \label{tab:navsafe_odyssey}
  \footnotesize
  \setlength{\tabcolsep}{3.4pt}
  \sbox0{%
  \resizebox{0.48\textwidth}{!}{%
  \begin{tabular}{lccccc}
    \toprule
    & & \multicolumn{2}{c}{NavSafe-$\infty$} & \multicolumn{2}{c}{Odyssey} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6}
    Method & Params. & DS $\uparrow$ & SR $\uparrow$ & NR $\uparrow$ & R $\uparrow$ \\
    \midrule
    LTF~\cite{chitta2023transfuser} & 56.0M & 53.0 & 27.7 & 20.1 & 23.0 \\
    DiffusionDrive~\cite{liao2025diffusiondrive} & 60.8M & 44.8 & 21.0 & 35.9 & 41.0 \\
    SafeDrive~\cite{kim2026safedrive} & -- & -- & -- & 44.4 & \underline{48.9} \\
    GTRS-Dense \simscale~\cite{li2025gtrs,tian2026simscale} & 81.0M & 73.5 & \underline{61.8} & -- & -- \\
    DrivoR~\cite{kirby2026drivor} & 40.8M & 64.7 & 50.7 & 36.5 & 41.4 \\
    DrivoR \simscale~\cite{kirby2026drivor,tian2026simscale} & 40.8M & 57.2 & 42.7 & 37.4 & 36.9 \\
    \rowcolor{argusrow} \argus & 31.7M & \underline{78.7} & \textbf{72.9} & \underline{48.8} & 47.2 \\
    \rowcolor{argusrow} \argusplus & 98.5M & \textbf{78.9} & \textbf{72.9} & \textbf{49.0} & \textbf{53.4} \\
    \bottomrule
  \end{tabular}}
  \unskip}\noindent\usebox0\par\vspace{2pt}\noindent
  \begin{minipage}{\wd0}\scriptsize\raggedright Baselines as published, gathered by \texttt{py123d\_garage}~\cite{kesai2026py123dgarage}.\par\end{minipage}%
\end{table}


==> tab/selfplay_extension_pai.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{Single-agent PPO on PAI}: AlpaSim score of \argusraster with its action head, after self-play only and after its extension to logged traffic, with mean progress and speed, rear-ended scenes, and failed scenes out of the 441 PAI validation scenes.}%
  \label{tab:selfplay_extension_pai}
  \scriptsize
  \setlength{\tabcolsep}{2.5pt}
  \begin{tabular}{@{}lccccccc@{}}
    \toprule
    & Score & Progress & Speed & Rear- & Colli- & Off- & Corridor \\
    & & (\%) & (m/s) & ended & sion & road & exit \\
    \midrule
    Self-play, w/~action & 61.1 & 61.6 & 8.9 & 147 & 24 & 7 & 23 \\
    + logged traffic, w/~action & 89.3 & 92.9 & 12.3 & 13 & 17 & 1 & 22 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tab/selfplay_pictura.tex <==
\begin{table}[t]%
  \centering
  \caption{\textbf{Self-play against \alberti.} The protocol of \pictura~\cite{yin2026pictura}: vehicle-only metrics, argmax. Self-play, w/~action: \argusraster after self-play only, before its extension to logged traffic, driving with its action head.
    Self-play on the CARLA maps at medium traffic density, with collision rate (Coll.), off-road rate (Off.), red-light violation rate (RLV), goals reached per agent (Goals), and km per infraction (km/inf.).
   }
  \label{tab:selfplay_pictura}
  \scriptsize
  \setlength{\tabcolsep}{4pt}
  \sbox0{%
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    Policy & Coll.\,$\downarrow$ & Off.\,$\downarrow$ & RLV\,$\downarrow$ & Goals\,$\uparrow$ & km/inf.\,$\uparrow$ \\
    \midrule
    \alberti~\cite{yin2026pictura} & 0.060 & 0.018 & 0.058 & 11.21 & 11.61 \\
    Self-play, w/~action & 0.002 & 0.003 & 0.002 & 8.68 & 105.90 \\
    \bottomrule
  \end{tabular}
  \unskip}\noindent\usebox0
\end{table}


==> tab/selfplay_rewards.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{Conditioning of \argusraster in self-play.}
    Coefficients of the reward terms of \autoref{sec:impl:selfplay} and dynamics multipliers, drawn per agent at every spawn in training and observed by the policy, and fixed in every evaluation.
    $\mathcal{X}(a) = \tfrac{1}{2}\,\mathcal{U}(1/a,1) + \tfrac{1}{2}\,\mathcal{U}(1,a)$.}
  \label{tab:selfplay_rewards}
  \footnotesize
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lll@{}}
    \toprule
    Coefficient & Training & Eval \\
    \midrule
    \multicolumn{3}{@{}l}{\textit{Reward}} \\
    Goal radius $\delta_\mathrm{goal}$ & $\mathcal{U}(2, 12)$\,m & 2\,m \\
    Goal speed $v_\mathrm{goal}$ & $\mathcal{U}(0, 40)$\,m/s & 40\,m/s \\
    Collision $\alpha_\mathrm{coll}$ & $\mathcal{U}(0, 3)$ & 3 \\
    Off-road $\alpha_\mathrm{off}$ & $\mathcal{U}(0, 3)$ & 3 \\
    Red light, stop sign $\alpha_\mathrm{stop}$ & $\mathcal{U}(0, 1)$ & 1 \\
    Lane alignment $\alpha_\mathrm{align}$ & $\mathcal{U}(2.5\cdot10^{-4}, 2.5\cdot10^{-2})$ & $2.5\cdot10^{-2}$ \\
    Wrong-way speed $\alpha_\mathrm{wrong}$ & $\mathcal{U}(0, 1)$ & 1 \\
    Lane centering $\alpha_\mathrm{center}$ & $\mathcal{U}(2.5\cdot10^{-4}, 7.5\cdot10^{-3})$ & $3.8\cdot10^{-3}$ \\
    Center bias $b$ & $\mathcal{U}(-0.5, 0.5)$\,m & 0 \\
    Comfort $\alpha_\mathrm{comf}$ & $\mathcal{U}(0, 10^{-1})$ & $5\cdot10^{-2}$ \\
    Overspeed $\alpha_\mathrm{over}$ & $\mathcal{U}(0, 1)$ & $5\cdot10^{-2}$ \\
    Reverse $\alpha_\mathrm{rev}$ & $\mathcal{U}(2.5\cdot10^{-4}, 7.5\cdot10^{-3})$ & $5\cdot10^{-3}$ \\
    Progress $\alpha_\mathrm{prog}$ & $2.5\cdot10^{-3}$ (fixed) & $2.5\cdot10^{-3}$ \\
    Time $\alpha_\mathrm{time}$ & $2.5\cdot10^{-5}$ (fixed) & $2.5\cdot10^{-5}$ \\
    \midrule
    \multicolumn{3}{@{}l}{\textit{Dynamics and speed}} \\
    Throttle multiplier $c_\mathrm{throttle}$ & $\mathcal{X}(1.25)$ & 1 \\
    Steering multiplier $c_\mathrm{steer}$ & $\mathcal{X}(1.25)$ & 1 \\
    Acceleration multiplier $c_\mathrm{acc}$ & $\mathcal{X}(1.5)$ & 1 \\
    Speed cap $v_\mathrm{max}$ & $40\,\mathcal{X}(1.5)$\,m/s & 40\,m/s \\%
    \bottomrule
  \end{tabular}
\end{table}


==> tab/training_settings.tex <==
\begin{table*}[t]
  \centering
  \caption{\textbf{Training settings}: hyperparameters of (a) the self-play of \argusraster and its extension to logged traffic, (b) the trajectory head of \argusraster, and (c) the alignment of \argus to \argusraster. $\tau$ is the fraction of a decay elapsed.}
  \label{tab:selfplay_hparams}\label{tab:logged_hparams}\label{tab:align_hparams}
  \scriptsize
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{0.95}
  \begin{minipage}[t]{0.49\textwidth}\centering
  (a) Self-play and its extension to logged traffic\par\smallskip
  \begin{tabular}{@{}>{\raggedright\arraybackslash}p{2.35cm}>{\raggedright\arraybackslash}p{2.5cm}>{\raggedright\arraybackslash}p{2.75cm}@{}}
    \toprule
    & Self-play & Extension to logged traffic \\
    \midrule
    \multicolumn{3}{@{}l}{\textit{Environment}} \\
    Scenes & 12 maps & 1{,}458 PAI + 12{,}861 navtrain \\
    Self-play world & on all environments & on 2 of 8 environments \\%
    Policy drives & every agent & the ego only \\%
    Step & 0.3\,s & 0.1\,s \\
    Episode & up to 750\,s & PAI 25\,s, navtrain 5.5\,s \\
    Goals & on the map's lanes & on the logged route \\%
    Ego dynamics & the simulator's & AlpaSim's \\%
    Cameras & a pool of rigs & the scene's (70\%), hood 50\% \\%
    \midrule
    \multicolumn{3}{@{}l}{\textit{Optimization}} \\
    $\gamma$, GAE $\lambda$~\cite{schulman2016gae} & 0.999, 0.95 & 0.999, 0.95 \\
    Clipping, value coefficient & 0.2, 0.5 & 0.2, 0.5 \\
    Entropy coefficient & 0.01 & 0.005 \\
    Gradient norm & 0.5 & 0.5 \\
    Epochs per update & 3 & 3 \\
    Rollout & 128 steps per agent & 128 steps per agent \\
    Samples per update & about 170M & -- \\
    Minibatch & 266{,}240 samples & 32{,}768 samples \\
    Advantage filtering & 0.01 $\times$ advantage EWMA & 0.01 $\times$ advantage EWMA \\
    Optimizer & AdamW, $\beta$ 0.9/0.999, w.d.\ 0.01 & AdamW, $\beta$ 0.9/0.999, w.d.\ 0.01 \\
    Learning rate & $5\cdot10^{-4}$, constant & $10^{-4}$, 3\% warmup \\
    Decay to 0 ($1-\sqrt{\tau}$) & over 10B more steps & over the last 50\% \\
    Critic alone, actor ramp & -- & first 12.5\%, then over 5\% \\
    Steps & 50B + 10B of decay & 342M, a quarter in self-play \\
    Hardware & 260 A100 GPUs, about 8\,h & 8 H100 GPUs, about 4\,h \\
    Precision & bfloat16 & bfloat16 \\
    \bottomrule
  \end{tabular}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.49\textwidth}\centering\renewcommand{\arraystretch}{1.075}%
  (b) Trajectory head of \argusraster\par\smallskip
  \begin{tabular}{@{}>{\raggedright\arraybackslash}p{2.35cm}>{\raggedright\arraybackslash}p{\dimexpr5.25cm+6pt\relax}@{}}%
    \toprule
    Scenes & the logged scenes of the training extension \\%
    Step, segments & 0.1\,s; 39 steps by the action head, then 21 by the trajectory head \\%
    Plan tracker & AlpaSim's linear MPC \\%
    Euler steps & 1 in training, 10 at deployment \\%
    Optimizer & AdamW, $2.5\cdot10^{-4}$, no warmup \\
    Decay & $1-\sqrt{\tau}$, over the last 30\% \\
    Steps & 256M in the logged scenes \\
    Hardware & 8 H100 GPUs, about 4\,h \\
    \bottomrule
  \end{tabular}
  \par\medskip
  (c) Alignment of \argus\par\smallskip
  \begin{tabular}{@{}>{\raggedright\arraybackslash}p{2.35cm}>{\raggedright\arraybackslash}p{\dimexpr5.25cm+6pt\relax}@{}}%
    \toprule
    \multicolumn{2}{@{}l}{\textit{Model}} \\
    Backbone & DINOv3 ViT-S/16, with ray codes \\
    LoRA & rank 32, all projections, w.d.\ 0.05 \\
    \midrule
    \multicolumn{2}{@{}l}{\textit{Data}} \\
    Scenes & PAI (NuRec) and navtrain (WorldEngine) \\%
    Drives & of \argusraster, with AlpaSim score 1 \\%
    Frames & PAI 313k, navtrain 580k \\
    Cameras & PAI: front, 2 cross (120$^\circ$), 2 rear (70$^\circ$), hood in, front telephoto out; navtrain: CAM\_F0, L0, R0, B0 of nuPlan \\
    Image size & resized to 1148$\times$672, center-cropped to 1136$\times$672 \\
    \midrule
    \multicolumn{2}{@{}l}{\textit{Optimization}} \\
    Optimizer & AdamW \\
    Learning rate & adapter $3\cdot10^{-4}$, LoRA $10^{-4}$ \\
    Schedule & 200 warmup steps, cosine decay \\
    Epochs, global batch & 20, 128 \\
    Hardware & 8 H100 GPUs, about 6\,h \\
    \bottomrule
  \end{tabular}
  \end{minipage}
\end{table*}

